No-brainer: Morphological Computation driven Adaptive Behavior in Soft Robots

It is prevalent in contemporary AI and robotics to separately postulate a brain modeled by neural networks and employ it to learn intelligent and adaptive behavior. While this method has worked very well for many types of tasks, it isn't the only type of intelligence that exists in nature. In this work, we study the ways in which intelligent behavior can be created without a separate and explicit brain for robot control, but rather solely as a result of the computation occurring within the physical body of a robot. Specifically, we show that adaptive and complex behavior can be created in voxel-based virtual soft robots by using simple reactive materials that actively change the shape of the robot, and thus its behavior, under different environmental cues. We demonstrate a proof of concept for the idea of closed-loop morphological computation, and show that in our implementation, it enables behavior mimicking logic gates, enabling us to demonstrate how such behaviors may be combined to build up more complex collective behaviors.

==> sections/related_work.tex <==
\textbf{Evolutionary Robotics} focuses on building intelligent agents from the bottom up by allowing evolution to optimize different parts of the agent. While evolution is allowed to alter more and more parts of the agents, the general approach is still to separately postulate a brain and body. Even when brains are evolved dependent on agents' bodies, either by explicitly conditioning the brains on body layout such as~\cite{sims_evolving_1994}
% {\color{blue}more citations of a nervous system evolving based on body layout}
or by implicitly relating brains and bodies with a single genome such as~\cite{bongard2003evolving},
% {\color{blue}more citations of the single genome for brain and body}
we study (usually implicitly) how the body could take part in the creation of intelligent behavior in tandem with a separately postulated brain. In this work instead, we study how adaptive and complex behavior can be created without a separately postulated brain. 

\textbf{Reinforcement Learning} is the study of algorithms to learn from experience. Specifically, deep reinforcement learning, where brains are modeled by neural networks and learned through backpropagation, has achieved great success~\cite{arulkumaran2017deep}. While the focus of the research is generally solely on the learning algorithms for the brain, recently we see an increasing interest in combining RL approaches with body optimization to further increase performance~\cite{gupta_embodied_2021}. We take a more extreme approach in this work and study how an agent could exhibit complex behavior without any brain.

\textbf{Braitenberg vehicles}~\cite{braitenberg1986vehicles} are one of the sources of inspiration for our work. It is a great example of how simple mechanisms give rise to complex behaviors. While early models of Braitenberg Vehicles come pre-equipped with tools to achieve the basic motor functionality (wheels to navigate), later vehicles progressively built a model of brain-like structure to demonstrate more complex behavior. In this work, instead, we focus on the creation of initial adaptive and complex sensory-motor behavior from basic building blocks.

\textbf{Granular meta-materials}~\cite{parsa2023universal}
% ~\cite{parsa2022evolving,parsa2022evolution,parsa2023universal,parsa2024gradient}
are shown to be capable of implementing logic gates and even computing multiple different logic operations at the same time and place. Here, we expand this research by circumventing the calculation of logical operations and directly turning the sensory input into the behavior of an agent by exploiting the system dynamics through optimization of the design of the robot morphology.

Specifically, we consider our work as the spiritual successor of previous research that examined morphological computation in planted, growing soft robots~\cite{corucci_material_2016}. Evolution optimizes the design of soft robots by placing voxels and determining their behavior according to the stimulus (expand or contract in response to stimulus) to minimize the distance towards the source of stimulus. When evolved soft robots are placed in an environment with stimulus, they grow (some voxels of the robot might shrink but the robot generally has to grow in order to reach a source) to extend part of their body towards a source. We follow a similar approach but instead of evolving extending behavior on planted-growing soft robots, we evolve robots to locomote. Moreover, we expect robots to adapt their behavior based on changing stimuli during their lifetime.
